Challenges in Designing Datasets and Validation for Autonomous Driving

Autonomous driving is getting a lot of attention in the last decade and will be the hot topic at least until the first successful certification of a car with Level 5 autonomy. There are many public datasets in the academic community. However, they are far away from what a robust industrial production system needs. There is a large gap between academic and industrial setting and a substantial way from a research prototype, built on public datasets, to a deployable solution which is a challenging task. In this paper, we focus on bad practices that often happen in the autonomous driving from an industrial deployment perspective. Data design deserves at least the same amount of attention as the model design. There is very little attention paid to these issues in the scientific community, and we hope this paper encourages better formalization of dataset design. More specifically, we focus on the datasets design and validation scheme for autonomous driving, where we would like to highlight the common problems, wrong assumptions, and steps towards avoiding them, as well as some open problems.

==> _tmp_/__nips_2017.tex <==


\section{Introduction} \label{sec:intro}
zz

% PK ideas - begin
Good data is key to everything, however this topic is often neglected. Data are difficult record, annotate and prepare. Often they are not i.i.d. for training, validation and testing.

Blindly using input data without looking at them. Blindly looking at result
 without understanding what could go wrong.Good spractice could be checking, e.g.,  miss-classified samples, or samples with the worse performance. This could recover problems with annotations, tools used to prepare the data, or tools to evaluate the performance.
% PK ideas - end

% DH - just blabbering a few ideas below - far from final text
Comparing models performance trained on different datasets is unfair and we can see it everywhere.

Almost all methods are compared just from the precision point of view (using some of standard metric - F-score, TPR, FPR, precision, ...). It is also essential to take into account the computational complexity of individual methods. Very often this aspect is completely ignored. When method A (high complexity) performs better than method B (low complexity) there is no guarantee that A would be still better when B would be used e.g. in cascaded form or in ensemble to reach overall complexity of method A.

In the machine learning research community, many topics are considered to be "solved". The reality is unfortunately completely different. The real world application task is much more challenging. The key to this lies in the datasets used for particular method development. The dataset represents the whole world and the training, validation and testing sets are nicely sampled from this dataset. Several methods are then compared and their performance boosted. One may get the impression that the real world problem also gets solved. There are attempts to evaluate on multiple datasets and get closer to the real world performance. This helps but still does not solve the problem of overfitting to datasets, which are far from becoming the real world sample. One example for all are low light evening/night captures which are nearly impossible to find among publicly available dataset. Also the requirements for precision in real applications are orders of magnitude higher than what is considered as solved problem among the researchers in machine learning community.
% ----------------- end DH blabber ------------------




\section{Dataset Design} \label{sec:dataset}
- Current datasets \\
- Design procedures \\
- Issues with current datasets \\
- Data Augmentation \\
- Synthetic Data \\

\section{Experimental Evaluation} \label{sec:experimental_eval}
\begin{itemize}
    \item Early decisions based on bad data (non-representative samples, small volume, \dots)
    \item 
\end{itemize}

\href{https://hci.iwr.uni-heidelberg.de/eccv16ws-datasets}{ECCV 2016 Workshop on Datasets and Performance Analysis in Early Vision}

\href{https://arxiv.org/pdf/1809.02492.pdf}{On the Importance of Visual Context for Data
Augmentation in Scene Understanding}

\href{https://arxiv.org/abs/1807.03341}{Troubling Trends in Machine Learning Scholarship}

\href{https://link.springer.com/article/10.1007/s11263-017-1020-z}{How Good Is My Test Data? Introducing Safety Analysis for Computer Vision}


\section{Validation} \label{sec:validation}
- Issues with standard loss function - class imabalance, diversity, etc \\
- KPI \\

\href{https://arxiv.org/pdf/1709.02435.pdf}{An Analysis of ISO 26262: Using Machine
Learning Safely in Automotive Software} \\

\href{https://www.researchgate.net/publication/320567319_Machine_Learning_Safety_An_Overview}{Machine Learning Safety: An Overview} \\

\href{http://mrksbrg.com/wp-content/uploads/preprints/2018_SEFAIAS_ISO26262.pdf}{Automotive safety and machine learning: Initial results from a
study on how to adapt the ISO 26262 safety standard} \\

\href{https://arxiv.org/pdf/1606.06565.pdf}{Concrete Problems in AI Safety} \\




Wild Patterns: Ten Years After the Rise of Adversarial Machine Learning \\
DeepXplore: Automated Whitebox Testingof Deep Learning Systems \\
DeepTest: Automated Testing ofDeep-Neural-Network-driven Autonomous Cars


\section{Conclusion} \label{sec:conc}
zz


{\small
\bibliographystyle{plain}
\bibliography{refs.bib}
}

\end{document}


==> include/macros.tex <==
\newcommand{\head}[1]{\par\medskip\noindent{\bf #1: }}
\newcommand{\rem}[1]{{\it \color{red} #1}}


%-- MMMakro ------------------                                                  
\def\##1{\relax\ifmmode\mathchoice      % italic bold vector, e.g. $\#{x}$
{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}\else
\hbox{\boldmath$\textstyle#1$}\fi}
\def\m#1{\mathbf{#1}}                  % bold matrix, e.g. $\m{A}$
%---------------------------------------

\def\dQ{\mathrm{d}Q}
\def\bar#1{\overline{#1}}

\def\Emph#1{\emph{#1}}
\def\Const#1{\mathrm{#1}}

\def\boxit#1{\vbox{\hrule\hbox{\vrule\vbox{\medskip\noindent#1                  
             \medskip}\vrule}\hrule}}                                           


\renewcommand{\Re}{\mathbb{R}}
\newcommand{\Ne}{\mathbb{N}}
\newcommand{\Na}{\mathbb{N}}
\newcommand{\FF}{\cal F}
\newcommand{\FX}{\cal X}
\newcommand{\FR}{\Re^n}
%\newcommand{\FS}{{S}}
%\newcommand{\dim}{\mathop dim}

\newcommand{\SG}{{\cal G}}
\newcommand{\SA}{{\cal A}}
\newcommand{\SB}{{\cal B}}
\newcommand{\SE}{{\cal E}}
\newcommand{\SF}{{\cal F}}
\newcommand{\SX}{{\cal X}}
\newcommand{\SCX}{\overline{\cal X}}
\newcommand{\SFX}{\tilde{\cal X}}
\newcommand{\SIsv}{{{\cal I}_{\emptyset}}}
\newcommand{\SY}{{\cal Y}}
\newcommand{\SZ}{{\cal Z}}
\newcommand{\ST}{{\cal T}}
\newcommand{\SH}{{\cal H}}
\newcommand{\SM}{{\cal M}}
\newcommand{\SC}{{\cal C}}
\newcommand{\sS}{{\cal S}}
\newcommand{\SP}{{\cal P}}
\newcommand{\SN}{{\cal N}}
\newcommand{\SW}{{\cal W}}
\newcommand{\Ssv}{{\cal S}}
\newcommand{\Ss}{{\cal S}}
\newcommand{\SQ}{{\cal Q}}
\newcommand{\SR}{\Re^n}
%\newcommand{\SI}{{\cal I}}
\newcommand{\SO}{{\cal O}}
\newcommand{\SJ}{{\cal J}}
\newcommand{\SL}{{\cal L}}
\newcommand{\SU}{{\cal U}}
\newcommand{\SD}{{\cal D}}
\newcommand{\SV}{{\cal V}}
\newcommand{\STheta}{\Theta}
\newcommand{\SSV}{{\cal I_{SV}}}

\newcommand{\eye}{\m{E}}
\newcommand{\one}{{\cal \m{1}}}
\newcommand{\nconst}{r}

\def\M3N{M$^3$N}


\def\kmse{\mathbb{\varepsilon}_{KMS}} 
\def\mse{\mathbb{\varepsilon}_{MS}} 
\def\qe{\mathbb{\varepsilon}_{QE}}
\def\rerr{\mathbb{\varepsilon}_{R}}
\def\tsterr{ \mathop{\rm TstErr}}
\def\nsv{ nsv }
\def\maxerr{\mathop{\rm \varepsilon_{max}}}
%\def\keval{\mathop{\rm KerEval}}
\def\keval{\mathop{\rm ker\_eval}}
\def\cputime{\mathop{ \rm CPU_{time}}}
\def\ls{\mathop{\rm \varepsilon_{LS}}}
\def\Err{ \mathop{\rm Err}}
\def\snr{\mathop{\rm SNR}}
\def\dontknow{\mathop{\rm dont\_know}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\equ#1{(\ref{#1})}

\def\veps{\varepsilon}
\def\Veps{\Varepsilon}

\def\lin{\mathop{\rm lin}}                                                
\def\argmax{\mathop{\rm argmax}}                                                
\def\Argmax{\mathop{\rm Argmax}} 
\def\argmin{\mathop{\rm argmin}}                                                
\def\Span{\mathop{\rm Span}}      
\def\Card{\mathop{\rm Card}}      
\def\Con{\mathop{\rm co}}
\def\diag{\mathop{\rm diag}}      
\def\sgn{\mathop{\rm sgn}}

\def\nm#1{\#\phi(#1)}
\def\tnm#1{\tilde{\#\phi}(#1)}
\def\tv#1{{\tilde{\##1}}}

\def\lz{\langle}
\def\pz{\rangle}

\def\det#1{\mathop{\rm det} ({#1} )}

\def\alphat{\#\alpha^{(t)}}
\def\clip{\mathop{\rm clip}}
\def\sgn{\mathop{\rm sgn}}

\def\leftbb{\mathopen{\rlap{$[$}\hskip1.3pt[}}
\def\rightbb{\mathclose{\rlap{$]$}\hskip1.3pt]}}
\def\ass{\mathrel {:=}}
\newcommand{\vphi}{\varphi}
\newcommand{\boldvphi}{\#\varphi}

\newcommand{\ldb}{\mathopen{\lbrack\!\lbrack}} 
\newcommand{\rdb}{\mathclose{\rbrack\!\rbrack}}

\newenvironment{suggestion}%
{%
\noindent\color{red}\textbf{Suggestion:}\\%
}%
{\par\noindent}


==> include/unfair_comparisons.tex <==
\section{(Un)Fair Comparisons} \label{sec:comparisons}


As a typical example of methods and models compared only from the performance point of view while ignoring the computational complexity we may take CNN vs. DPM (older but very successful Deformable Part Models \cite{felzenswalb2010}). Usually we see stronger CNN beating DPM but at what computational cost? As a counter example we did a comparison of equally complex models with the same number of operations (as similar as possible) during inference. Please see testing set results on Figure~\ref{fig:dpm}, where we experimented with these methods on our internal pedestrian dataset in real driving scenarios. No surprise that DPM beats CNN in multiple settings. Both methods were trained on the same training data with an attempt to reach i.i.d. sampling (for both training and testing sets).

\begin{figure}[tbh]
    \centering
    \includegraphics[width=\linewidth]{Images/dpm.png}
    \caption{Performance comparison for equally complex CNN and DPM models on a pedestrian detection task. Multiple settings were tested in an attempt to reach best performance for both methods. Due to internal confidentiality rules we can not reveal individual settings. Here only SVM+HOG had lower complexity than other models and served as a baseline.}
    \label{fig:dpm}
\end{figure}
